An eclipsing binary black hole candidate system in the blazar Mrk 421

Removing outbursts from multiwavelength light curves of the blazar Mrk~421, we construct outburstless time series for this system. A model-independent power spectrum light curve analysis in the optical, hard X-ray and gamma-rays for this outburstless state and also the full light-curves, show clear evidence for a periodicity of ~ 310 days across all wavelengths studied. A subsequent full maximum likelihood analysis fitting an eclipse model confirms a periodicity of 310 \pm 1 days. The power spectrum of the signal in the outburstless state of the source does not follow a flicker noise behaviour and so, the system producing it is not self-organised. This and the fact that the periodicity is better defined in the outburstless state, strongly suggests that it is not produced by any internal physical processes associated to the central engine. The simplest physical mechanism to which this periodicity could be ascribed is a dynamical effect produced by an orbiting supermassive black hole companion eclipsing the central engine. Interestingly, the optimal eclipse model infers a brightness enhancement of (136.4 \pm 20 )%, suggesting an eclipse resulting in a gravitational lensing brightening. Consisting with this interpretation, the eclipse occurs for only ( 9.7 \pm 0.2)% of the orbital period.

==> aas-journals.tex <==
% This file should be included on a main document with an \include option. 
% 
% This is what the AAS defines for bibtex entries.  This file was downloaded
% from the ADS Database (Simbad) here:
% http://adsabs.harvard.edu/abs_doc/aas_macros.html
% 
%   In order to use it go to the ads and ask for a bibtex entry of your
% favourite article...
% 
% Sergio Mendoza
% Cavendish Labs
% Cambridge UK
% Tue Mar 14 20:30:18 GMT 2000
% 
\newcommand{\aj}{Astronomical Journal}
\newcommand{\araa}{Ann. Rev. Ast. \& Ast.}
% \newcommand{\apj}{ApJ}
\newcommand{\apj}{Astrophysical Journal}
\newcommand{\apjl}{ApJL}
\newcommand{\apjs}{ApJS}
% \newcommand{\ao}{Applied Optics}
\newcommand{\apss}{Astrophysics and Space Science}
\newcommand{\aap}{Astronomy and Astrophysics}
\newcommand{\aapr}{Astronomy and Astrophysics Reviews}
\newcommand{\aaps}{Astronomy and Astrophysics, Supplement}
\newcommand{\azh}{Astronomicheskii Zhurnal}
\newcommand{\baas}{Bulletin of the AAS}
\newcommand{\jcap}{Journal of Cosmology and Astroparticle Physics}
\newcommand{\jrasc}{Journal of the RAS of Canada}
\newcommand{\memras}{Memoirs of the RAS}
%\newcommand{\mnras}{Monthly Notices of the RAS}
\newcommand{\mnras}{MNRAS}
% \newcommand{\pra}{Physical Review A: General Physics}
% \newcommand{\prb}{Physical Review B: Solid State}
% \newcommand{\prc}{Physical Review C}
% \newcommand{\prd}{Physical Review D}
% \newcommand{\pre}{Physical Review E}
% \newcommand{\prl}{Physical Review Letters}
\newcommand{\pasp}{Publications of the ASP}
\newcommand{\pasj}{Publications of the ASJ}
\newcommand{\qjras}{Quarterly Journal of the RAS}
\newcommand{\skytel}{Sky and Telescope}
\newcommand{\solphys}{Solar Physics}
\newcommand{\sovast}{Soviet Astronomy}
\newcommand{\ssr}{Space Science Reviews}
\newcommand{\zap}{Zeitschrift fuer Astrophysik}
% \newcommand{\nat}{Nature}
\newcommand{\iaucirc}{IAU Cirulars}
\newcommand{\aplett}{Astrophysics Letters}
\newcommand{\apspr}{Astrophysics Space Physics Research}
\newcommand{\bain}{Bulletin Astronomical Institute of the Netherlands}
\newcommand{\fcp}{Fundamental Cosmic Physics}
\newcommand{\gca}{Geochimica Cosmochimica Acta}
\newcommand{\grl}{Geophysics Research Letters}
% \newcommand{\jcp}{Journal of Chemical Physics}
\newcommand{\jgr}{Journal of Geophysics Research}
\newcommand{\jqsrt}{Journal of Quantitiative Spectroscopy and Radiative Transfer}
\newcommand{\memsai}{Mem. Societa Astronomica Italiana}
\newcommand{\nphysa}{Nuclear Physics A}
\newcommand{\physrep}{Physics Reports}
\newcommand{\physscr}{Physica Scripta}
\newcommand{\planss}{Planetary Space Science}
\newcommand{\procspie}{Proceedings of the SPIE}


